ILLUMINER: Instruction-tuned Large Language Models as Few-shot Intent Classifier and Slot Filler

State-of-the-art intent classification (IC) and slot filling (SF) methods often rely on data-intensive deep learning models, limiting their practicality for industry applications. Large language models on the other hand, particularly instruction-tuned models (Instruct-LLMs), exhibit remarkable zero-shot performance across various natural language tasks. This study evaluates Instruct-LLMs on popular benchmark datasets for IC and SF, emphasizing their capacity to learn from fewer examples. We introduce ILLUMINER, an approach framing IC and SF as language generation tasks for Instruct-LLMs, with a more efficient SF-prompting method compared to prior work. A comprehensive comparison with multiple baselines shows that our approach, using the FLAN-T5 11B model, outperforms the state-of-the-art joint IC+SF method and in-context learning with GPT3.5 (175B), particularly in slot filling by 11.1--32.2 percentage points. Additionally, our in-depth ablation study demonstrates that parameter-efficient fine-tuning requires less than 6% of training data to yield comparable performance with traditional full-weight fine-tuning.

==> related_old.tex <==
\paragraph{Prior Work on IC, SF, DST}
The following papers mainly focused on using LLMs for the Dialogue State Tracking (DST), Intent Classification (IC) and Slot Filling (SF) tasks. A survey paper about recent approaches for DST \cite{jacqmin-etal-2022-follow} provided a brief overview about existing work leveraging the prompting-generative-models approach. In order to improve pretrained LMs for the abovementioned tasks, \citet{wang-etal-2022-deepstruct} proposed the task-adaptation finetuning for the more general task of structure prediction.

The difference between DST and SF is that in DST, the goal is to do SF for all turns in a dialogue, which can be interdependent. Meanwhile, SF focus more on the information extraction from a single user utterance.

\paragraph{Dialogue State Tracking} Prior work mostly used MultiWoz \cite{dey-etal-2022-towards,wang-etal-2022-slot,hu-etal-2022-context,su2022selective,gupta-etal-2022-show,won-etal-2023-break,bang-etal-2023-task,aksu-etal-2023-prompter}, SGD \cite{DBLP:conf/aaai/RastogiZSGK20,sreedhar-parisien-2022-prompt} or both \cite{hudeček2023llms}.

\paragraph{Slot Filling} The most popular datasets for the slot filling task include SNIPS \cite{li-etal-2023-generative,Yang_Zhou_Yang_Ma_Dong_Atawulla_2023} and ATIS \cite{basu-etal-2022-strategies}. An industry-track paper used Amazon MASSIVE \cite{parikh-etal-2023-exploring}.
